A SAT-based Public Key Cryptography Scheme

A homomorphic public key crypto-scheme based on the Boolean Satisfiability Problem is proposed. The public key is a SAT formula satisfied by the private key. Probabilistic encryption generates functions implied to be false by the public key XOR the message bits. A zero-knowledge proof is used to provide signatures.

==> plots.tex <==
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%




\begin{figure*}[hbp]
\centering
\begin{minipage}{0.49\textwidth}
\centering
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1307){\makebox(0,0)[r]{\strut{}$2^{-10}$}}%
      \put(726,2159){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(726,3012){\makebox(0,0)[r]{\strut{}1}}%
      \put(726,3864){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(726,4717){\makebox(0,0)[r]{\strut{}$2^{10}$}}%
      \put(858,1034){\makebox(0,0){\strut{} 300}}%
      \put(1615,1034){\makebox(0,0){\strut{} 400}}%
      \put(2372,1034){\makebox(0,0){\strut{} 500}}%
      \put(3129,1034){\makebox(0,0){\strut{} 600}}%
      \put(3886,1034){\makebox(0,0){\strut{} 700}}%
      \put(4643,1034){\makebox(0,0){\strut{} 800}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2750,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3247,393){\makebox(0,0)[r]{\strut{}$2^{-13 + 0.033 n}$}}%
      \csname LTb\endcsname%
      \put(3247,173){\makebox(0,0)[r]{\strut{}$2^{-22 + 0.036 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench4_3}}%
    \gplfronttext
  \end{picture}%
\caption{
MiniSat run times for $m/n=4.3$.
\label{fig:k3r4.3}}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\centering
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1938){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(594,2706){\makebox(0,0)[r]{\strut{}1}}%
      \put(594,3474){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(594,4242){\makebox(0,0)[r]{\strut{}$2^{10}$}}%
      \put(594,5011){\makebox(0,0)[r]{\strut{}$2^{15}$}}%
      \put(726,1034){\makebox(0,0){\strut{} 200}}%
      \put(1509,1034){\makebox(0,0){\strut{} 300}}%
      \put(2293,1034){\makebox(0,0){\strut{} 400}}%
      \put(3076,1034){\makebox(0,0){\strut{} 500}}%
      \put(3860,1034){\makebox(0,0){\strut{} 600}}%
      \put(4643,1034){\makebox(0,0){\strut{} 700}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2684,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3181,393){\makebox(0,0)[r]{\strut{}$2^{-14 + 0.042 n}$}}%
      \csname LTb\endcsname%
      \put(3181,173){\makebox(0,0)[r]{\strut{}$2^{-18 + 0.032 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench4_5}}%
    \gplfronttext
  \end{picture}%
\caption{
MiniSat run times for $m/n=4.5$.
\label{fig:k3r4.5}}
\end{minipage}
\end{figure*}


\begin{figure*}[hbp]
%\plotBenchF
\centering
\begin{minipage}{0.49\textwidth}
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
\centering
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1342){\makebox(0,0)[r]{\strut{}$2^{-10}$}}%
      \put(726,1984){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(726,2625){\makebox(0,0)[r]{\strut{}1}}%
      \put(726,3266){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(726,3908){\makebox(0,0)[r]{\strut{}$2^{10}$}}%
      \put(726,4549){\makebox(0,0)[r]{\strut{}$2^{15}$}}%
      \put(726,5191){\makebox(0,0)[r]{\strut{}$2^{20}$}}%
      \put(858,1034){\makebox(0,0){\strut{} 200}}%
      \put(1615,1034){\makebox(0,0){\strut{} 300}}%
      \put(2372,1034){\makebox(0,0){\strut{} 400}}%
      \put(3129,1034){\makebox(0,0){\strut{} 500}}%
      \put(3886,1034){\makebox(0,0){\strut{} 600}}%
      \put(4643,1034){\makebox(0,0){\strut{} 700}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2750,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3247,393){\makebox(0,0)[r]{\strut{}$2^{-18 + 0.061 n}$}}%
      \csname LTb\endcsname%
      \put(3247,173){\makebox(0,0)[r]{\strut{}$2^{-23 + 0.056 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench5_0}}%
    \gplfronttext
  \end{picture}%
\caption{MiniSat run times for $m/n=5$.
\label{fig:k3r5}}
\end{minipage}
\begin{minipage}{0.49\textwidth}
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
\centering
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,2032){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(594,3082){\makebox(0,0)[r]{\strut{}1}}%
      \put(594,4132){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(594,5182){\makebox(0,0)[r]{\strut{}$2^{10}$}}%
      \put(726,1034){\makebox(0,0){\strut{} 200}}%
      \put(1705,1034){\makebox(0,0){\strut{} 300}}%
      \put(2685,1034){\makebox(0,0){\strut{} 400}}%
      \put(3664,1034){\makebox(0,0){\strut{} 500}}%
      \put(4643,1034){\makebox(0,0){\strut{} 600}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2684,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3181,393){\makebox(0,0)[r]{\strut{}$2^{-16 + 0.047 n}$}}%
      \csname LTb\endcsname%
      \put(3181,173){\makebox(0,0)[r]{\strut{}$2^{-21 + 0.049 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench6_0}}%
    \gplfronttext
  \end{picture}%
\caption{
MiniSat run times for $m/n=6$.
\label{fig:k3r6}}
\end{minipage}
\end{figure*}

\begin{figure*}[hbp]
\centering
\begin{minipage}{0.49\textwidth}
\centering
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1568){\makebox(0,0)[r]{\strut{}$2^{-10}$}}%
      \put(726,2634){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(726,3700){\makebox(0,0)[r]{\strut{}1}}%
      \put(726,4767){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(858,1034){\makebox(0,0){\strut{} 200}}%
      \put(1804,1034){\makebox(0,0){\strut{} 300}}%
      \put(2751,1034){\makebox(0,0){\strut{} 400}}%
      \put(3697,1034){\makebox(0,0){\strut{} 500}}%
      \put(4643,1034){\makebox(0,0){\strut{} 600}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2750,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3247,393){\makebox(0,0)[r]{\strut{}$2^{-16 + 0.04 n}$}}%
      \csname LTb\endcsname%
      \put(3247,173){\makebox(0,0)[r]{\strut{}$2^{-23 + 0.046 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench7_0}}%
    \gplfronttext
  \end{picture}%
\caption{MiniSat run times for $m/n=7$.
\label{fig:k3r7}}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\centering
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \begin{picture}(5040.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,2021){\makebox(0,0)[r]{\strut{}$2^{-5}$}}%
      \put(594,2934){\makebox(0,0)[r]{\strut{}1}}%
      \put(594,3847){\makebox(0,0)[r]{\strut{}$2^5$}}%
      \put(594,4760){\makebox(0,0)[r]{\strut{}$2^{10}$}}%
      \put(726,1034){\makebox(0,0){\strut{} 200}}%
      \put(1286,1034){\makebox(0,0){\strut{} 300}}%
      \put(1845,1034){\makebox(0,0){\strut{} 400}}%
      \put(2405,1034){\makebox(0,0){\strut{} 500}}%
      \put(2964,1034){\makebox(0,0){\strut{} 600}}%
      \put(3524,1034){\makebox(0,0){\strut{} 700}}%
      \put(4083,1034){\makebox(0,0){\strut{} 800}}%
      \put(4643,1034){\makebox(0,0){\strut{} 900}}%
      \put(220,3374){\rotatebox{-270}{\makebox(0,0){\strut{}CPU time [s]}}}%
      \put(2684,814){\makebox(0,0){\strut{}$n$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3181,393){\makebox(0,0)[r]{\strut{}$2^{-15 + 0.032 n}$}}%
      \csname LTb\endcsname%
      \put(3181,173){\makebox(0,0)[r]{\strut{}$2^{-17 + 0.031 n}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{bench8_0}}%
    \gplfronttext
  \end{picture}%

\caption{MiniSat run times for $m/n=8$.
\label{fig:k3r8}}
\end{minipage}
\end{figure*}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ses-kryptoSAT"
%%% End: 

